Beyond Random Augmentations: Pretraining with Hard Views

Self-Supervised Learning (SSL) methods typically rely on random image augmentations, or views, to make models invariant to different transformations. We hypothesize that the efficacy of pretraining pipelines based on conventional random view sampling can be enhanced by explicitly selecting views that benefit the learning progress. A simple yet effective approach is to select hard views that yield a higher loss. In this paper, we propose Hard View Pretraining (HVP), a learning-free strategy that extends random view generation by exposing models to more challenging samples during SSL pretraining. HVP encompasses the following iterative steps: 1) randomly sample multiple views and forward each view through the pretrained model, 2) create pairs of two views and compute their loss, 3) adversarially select the pair yielding the highest loss according to the current model state, and 4) perform a backward pass with the selected pair. In contrast to existing hard view literature, we are the first to demonstrate hard view pretraining's effectiveness at scale, particularly training on the full ImageNet-1k dataset, and evaluating across multiple SSL methods, ConvNets, and ViTs. As a result, HVP sets a new state-of-the-art on DINO ViT-B/16, reaching 78.8% linear evaluation accuracy (a 0.6% improvement) and consistent gains of 1% for both 100 and 300 epoch pretraining, with similar improvements across transfer tasks in DINO, SimSiam, iBOT, and SimCLR.

==> algorithms/algorithm_nowrap.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
\caption{Pretraining with Hard Views}\label{alg}
\setlength{\itemsep}{-0.1ex}
\STATE \textbf{Input:} Number of views $N \geq 2$, batch size $M$, 
\STATE augmentation distribution \(\mathcal{T}\), encoder \(f_{\theta}\), projector \(g_{\theta}\)
\FOR{each $x_i$ in the sampled minibatch \(\left\{x_i\right\}_{i=1}^M\)}
    \STATE Sample $N$ augmentations: $A=\left\{t_n \sim \mathcal{T} \right\}_{n=0}^N$
    \STATE Create augmented views: $\textbf{x}_i^{A}= \left\{t_n(x_i)\right\}_{n=0}^N$ 
    \STATE Forward all views through $f_{\theta}$ and $g_{\theta}$ to get $z$ and $h$
    \STATE Create all $\binom{N}{2}$ possible pairs $\textbf{x}_i^{A_k} \times \textbf{x}_i^{A_l}$, $k \neq l$
    
    %\State For all pairs $(x_i^{A_k}, x_i^{A_l})$ forward through $f_{\theta}$ and $g_{\theta}$
    
    \STATE Select the \emph{hard} pair $(x_i^{A_{k_*}}, x_i^{A_{l_*}})$ maximizing Eq. \ref{eq:acl}
\ENDFOR
    \STATE Create the minibatch $(\textbf{x}^{A_{k_*}}, \textbf{x}^{A_{l_*}})$ of hard pairs 
    \STATE Proceed with standard discriminative SSL training\newline to 
    update \(\theta\) with the hard batch
    \STATE Repeat for all minibatches
\STATE \textbf{return} Optimized \(\theta\)

\end{algorithmic}
\end{algorithm}
%\vspace{-1em}

==> tables/13_merged.tex <==
\begin{table}[h]
    \centering
    \tabcolsep=0.10cm
    \footnotesize
    \begin{tabular}{llllll}
        \toprule
        Res. & SimSiam (RN50) & DINO (ViT) & Method & Arch. & Lin. \\
        \midrule
        100\% & x1.55 & x2.15 & DINO & ViT-S/16 & 74.06 \\
        75\% & x1.45 & x1.68 & DINO + HVS & ViT-S/16 & 74.67 \\
        50\% & x1.24 & x1.56 & \textbf{Improvement} & & \textbf{+0.61} \\
        25\% & x1.16 & x1.5 & \\ % <-- added \\ here
        \midrule
        & & & SimSiam & RN50 & 68.46 \\
        & & & SimSiam + HVS & RN50 & 68.98 \\
        & & & \textbf{Improvement} & & \textbf{+0.52} \\
        \midrule
        & & & SimCLR & RN50 & 64.31 \\
        & & & SimCLR + HVS & RN50 & 65.33 \\
        & & & \textbf{Improvement} & & \textbf{+1.02} \\
        \bottomrule
    \end{tabular}
    \caption{Time slowdown factors under different image resolutions and normalized performance.}
    \label{tab:merged_table}
\end{table}


==> tables/14_fig1_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{siunitx} % Add this package for better number alignment
\begin{table*}[ht]
\centering
\begin{tabular}{@{}SSSS@{}}
\toprule
\multicolumn{2}{c}{\textbf{Epoch}} & \multicolumn{2}{c}{\textbf{L.E. Acc.}} \\ \cmidrule(lr){1-2} \cmidrule(lr){3-4} 
{DINO+HVP} & {DINO} & {DINO+HVP} & {DINO} \\ \midrule
67  & 100 & 74.23 & 73.50 \\
100 & {-} & 74.67 & {-}   \\
200 & 300 & 75.30 & 75.50 \\
300 & {-} & 76.56 & {-}   \\
%{-} & 500 & {-}   & 76.05 \\
400 & 600 & {running} & 76.13 \\ \bottomrule
\end{tabular}
\caption{Performance and epoch values for DINO comparison figure.}
\label{tab:fig1_table}
\end{table*}


